ConvMambaNet: A Hybrid CNN-Mamba State Space Architecture for Accurate and Real-Time EEG Seizure Detection

Epilepsy is a chronic neurological disorder marked by recurrent seizures that can severely impact quality of life. Electroencephalography (EEG) remains the primary tool for monitoring neural activity and detecting seizures, yet automated analysis remains challenging due to the temporal complexity of EEG signals. This study introduces ConvMambaNet, a hybrid deep learning model that integrates Convolutional Neural Networks (CNNs) with the Mamba Structured State Space Model (SSM) to enhance temporal feature extraction. By embedding the Mamba-SSM block within a CNN framework, the model effectively captures both spatial and long-range temporal dynamics. Evaluated on the CHB-MIT Scalp EEG dataset, ConvMambaNet achieved a 99% accuracy and demonstrated robust performance under severe class imbalance. These results underscore the model's potential for precise and efficient seizure detection, offering a viable path toward real-time, automated epilepsy monitoring in clinical environments.

==> legend.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp3965714253297634] 
\draw  [color={rgb, 255:red, 240; green, 240; blue, 240 }  ,draw opacity=1 ][fill={rgb, 255:red, 240; green, 240; blue, 240}  ,fill opacity=1 ] (49.75,28.67) -- (234.5,28.67) -- (234.5,50) -- (49.75,50) -- cycle ;
%Straight Lines [id:da35709816095985714] 
\draw [color={rgb, 255:red, 52; green, 138; blue, 189 }  ,draw opacity=1 ][fill={rgb, 255:red, 49; green, 177; blue, 148 }  ,fill opacity=1 ][line width=1]    (141,40) -- (176.56,40.11) ;
%Straight Lines [id:da21073186915218378] 
\draw [color={rgb, 255:red, 226; green, 74; blue, 51 }  ,draw opacity=1 ][line width=1]    (56,40) -- (91.56,40.11) ;

% Text Node
\draw (92.22,35) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize] [align=left] {{\footnotesize Training}};
% Text Node
\draw (177.22,35) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize Validation}};


\end{tikzpicture}

